Stereo DSO: Large-Scale Direct Sparse Visual Odometry with Stereo Cameras

We propose Stereo Direct Sparse Odometry (Stereo DSO) as a novel method for highly accurate real-time visual odometry estimation of large-scale environments from stereo cameras. It jointly optimizes for all the model parameters within the active window, including the intrinsic/extrinsic camera parameters of all keyframes and the depth values of all selected pixels. In particular, we propose a novel approach to integrate constraints from static stereo into the bundle adjustment pipeline of temporal multi-view stereo. Real-time optimization is realized by sampling pixels uniformly from image regions with sufficient intensity gradient. Fixed-baseline stereo resolves scale drift. It also reduces the sensitivities to large optical flow and to rolling shutter effect which are known shortcomings of direct image alignment methods. Quantitative evaluation demonstrates that the proposed Stereo DSO outperforms existing state-of-the-art visual odometry methods both in terms of tracking accuracy and robustness. Moreover, our method delivers a more precise metric 3D reconstruction than previous dense/semi-dense direct approaches while providing a higher reconstruction density than feature-based methods.

==> RelatedWork.tex <==
\section{Related Work}
Feature-based VO was initially addressed by filtering approaches~\cite{chiuso2002structure, davison2007monoslam, civera2008inverse}.
Then more research effort has been put onto the keyframe-based approaches as mapping only needs to be performed on selected frames and thus more sophisticated optimization can be applied.
One example is PTAM~\cite{klein2007parallel} that parallelizes the optimization for tracking and mapping.
The Keyframe-based framework has been further developed by Strasdat \etal to integrate scale~\cite{strasdat2010scale} and then into a double window optimization pipeline~\cite{strasdat2011double}.
A more recent feature-based method ORB-SLAM~\cite{mur2015orb, mur2016orb} has gained a lot of popularity due to its high tracking accuracy and robustness, as well as several other nice features like loop closure and map reuse.
It has achieved state-of-the-art performance on several datasets such as the KITTI Dataset~\cite{geiger2013vision} and the EuRoc MAV Dataset~\cite{burri2016euroc}.
We compare the performance of our method with ORB-SLAM in Sec~\ref{sec:evaluation}.

Direct VO methods try to estimate camera poses by minimizing the photometric error from image alignment. 
The optimization is performed directly on pixel intensities instead of cautiously designed features, therefore more information from the images can be used.
The direct concept has been successfully applied for RGB-D images in~\cite{kerl2013dense, kerl2013robust, klose2013efficient}. 
With the given depth images, high tracking robustness and efficiency can be achieved.
On RGB images, direct image alignment is combined with a variational formulation to deliver dense 3D reconstructions~\cite{stuhmer2010real, newcombe2011dtam}. 
Since entire images are used, these computationally expensive approaches are usually limited to run in small workspace or on powerful GPUs. 
A semi-dense VO method has been proposed in~\cite{engel2013semi} to reduce the computational burden by only using pixels with high intensity gradient.
Geometric and photometric errors are minimized for the selected pixels which enables real-time VO on CPUs and even on smart phones~\cite{schops2014semi}.
This novel approach has been later extended to the popular LSD-SLAM system~\cite{engel2014lsd,engel2015large}. 
By integrating pose graph optimization, the system constructs a semi-dense 3D map with global consistency. 
Since then, the semi-dense direct VO/SLAM has been further developed for omnidirectional cameras~\cite{caruso2015large} and with IMU integration~\cite{usenko2016direct}.
A rolling shutter calibration method for LSD-SLAM has been recently proposed in~\cite{kim2016direct}.
The most recent direct VO method is proposed in~\cite{engel2016direct}.
With a evenly selected sparse pixel set, the monocular VO method performs a joint optimization for all model parameters and achieves unprecedented tracking accuracy. 
The method requires a full photometric calibration for which the camera response function, the dense lens vignetting factor, as well as the exposure time for each frame need to be available.
To the best of our knowledge, ~\cite{engel2016monodataset} is currently the only dataset that provides such information.
In this work we propose a novel formulation to integrate stereo cameras to the system, which highly increases the accuracy and robustness on images without photometric calibration.
The performance is evaluated on three widely used datasets in Sec~\ref{sec:evaluation}. 

